CATCH: a Cost Analysis Tool for Co-optimization of chiplet-based Heterogeneous systems

With the increasing prevalence of chiplet systems in high-performance computing applications, the number of design options has increased dramatically. Instead of chips defaulting to a single die design, now there are options for 2.5D and 3D stacking along with a plethora of choices regarding configurations and processes. For chiplet-based designs, high-impact decisions such as those regarding the number of chiplets, the design partitions, the interconnect types, and other factors must be made early in the development process. In this work, we describe an open-source tool, CATCH, that can be used to guide these early design choices. We also present case studies showing some of the insights we can draw by using this tool. We look at case studies on optimal chip size, defect density, test cost, IO types, assembly processes, and substrates.

==> DATE_submission.tex <==
% %% bare_conf.tex
% %% V1.4b
% %% 2015/08/26
% %% by Michael Shell
% %% See:
% %% http://www.michaelshell.org/
% %% for current contact information.
% %%
% %% This is a skeleton file demonstrating the use of IEEEtran.cls
% %% (requires IEEEtran.cls version 1.8b or later) with an IEEE
% %% conference paper.
% %%
% %% Support sites:
% %% http://www.michaelshell.org/tex/ieeetran/
% %% http://www.ctan.org/pkg/ieeetran
% %% and
% %% http://www.ieee.org/

% %%*************************************************************************
% %% Legal Notice:
% %% This code is offered as-is without any warranty either expressed or
% %% implied; without even the implied warranty of MERCHANTABILITY or
% %% FITNESS FOR A PARTICULAR PURPOSE! 
% %% User assumes all risk.
% %% In no event shall the IEEE or any contributor to this code be liable for
% %% any damages or losses, including, but not limited to, incidental,
% %% consequential, or any other damages, resulting from the use or misuse
% %% of any information contained here.
% %%
% %% All comments are the opinions of their respective authors and are not
% %% necessarily endorsed by the IEEE.
% %%
% %% This work is distributed under the LaTeX Project Public License (LPPL)
% %% ( http://www.latex-project.org/ ) version 1.3, and may be freely used,
% %% distributed and modified. A copy of the LPPL, version 1.3, is included
% %% in the base LaTeX documentation of all distributions of LaTeX released
% %% 2003/12/01 or later.
% %% Retain all contribution notices and credits.
% %% ** Modified files should be clearly indicated as such, including  **
% %% ** renaming them and changing author support contact information. **
% %%*************************************************************************


% % *** Authors should verify (and, if needed, correct) their LaTeX system  ***
% % *** with the testflow diagnostic prior to trusting their LaTeX platform ***
% % *** with production work. The IEEE's font choices and paper sizes can   ***
% % *** trigger bugs that do not appear when using other class files.       ***                          ***
% % The testflow support page is at:
% % http://www.michaelshell.org/tex/testflow/



% \documentclass[conference]{IEEEtran}
% % Some Computer Society conferences also require the compsoc mode option,
% % but others use the standard conference format.
% %
% % If IEEEtran.cls has not been installed into the LaTeX system files,
% % manually specify the path to it like:
% % \documentclass[conference]{../sty/IEEEtran}


% \usepackage{fancyhdr}


% % Some very useful LaTeX packages include:
% % (uncomment the ones you want to load)


% % *** MISC UTILITY PACKAGES ***
% %
% %\usepackage{ifpdf}
% % Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% % compilation based on whether the output is pdf or dvi.
% % usage:
% % \ifpdf
% %   % pdf code
% % \else
% %   % dvi code
% % \fi
% % The latest version of ifpdf.sty can be obtained from:
% % http://www.ctan.org/pkg/ifpdf
% % Also, note that IEEEtran.cls V1.7 and later provides a builtin
% % \ifCLASSINFOpdf conditional that works the same way.
% % When switching from latex to pdflatex and vice-versa, the compiler may
% % have to be run twice to clear warning/error messages.






% % *** CITATION PACKAGES ***
% %
% %\usepackage{cite}
% % cite.sty was written by Donald Arseneau
% % V1.6 and later of IEEEtran pre-defines the format of the cite.sty package
% % \cite{} output to follow that of the IEEE. Loading the cite package will
% % result in citation numbers being automatically sorted and properly
% % "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using
% % cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's
% % \cite will automatically add leading space, if needed. Use cite.sty's
% % noadjust option (cite.sty V3.8 and later) if you want to turn this off
% % such as if a citation ever needs to be enclosed in parenthesis.
% % cite.sty is already installed on most LaTeX systems. Be sure and use
% % version 5.0 (2009-03-20) and later if using hyperref.sty.
% % The latest version can be obtained at:
% % http://www.ctan.org/pkg/cite
% % The documentation is contained in the cite.sty file itself.





% \usepackage{soul}
% \usepackage{color}
% \usepackage{amsmath}
% \usepackage{graphicx}
% % *** GRAPHICS RELATED PACKAGES ***
% %
% \ifCLASSINFOpdf
%   % \usepackage[pdftex]{graphicx}
%   % declare the path(s) where your graphic files are
%   % \graphicspath{{../pdf/}{../jpeg/}}
%   % and their extensions so you won't have to specify these with
%   % every instance of \includegraphics
%   % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
% \else
%   % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
%   % will default to the driver specified in the system graphics.cfg if no
%   % driver is specified.
%   % \usepackage[dvips]{graphicx}
%   % declare the path(s) where your graphic files are
%   % \graphicspath{{../eps/}}
%   % and their extensions so you won't have to specify these with
%   % every instance of \includegraphics
%   % \DeclareGraphicsExtensions{.eps}
% \fi
% % graphicx was written by David Carlisle and Sebastian Rahtz. It is
% % required if you want graphics, photos, etc. graphicx.sty is already
% % installed on most LaTeX systems. The latest version and documentation
% % can be obtained at: 
% % http://www.ctan.org/pkg/graphicx
% % Another good source of documentation is "Using Imported Graphics in
% % LaTeX2e" by Keith Reckdahl which can be found at:
% % http://www.ctan.org/pkg/epslatex
% %
% % latex, and pdflatex in dvi mode, support graphics in encapsulated
% % postscript (.eps) format. pdflatex in pdf mode supports graphics
% % in .pdf, .jpeg, .png and .mps (metapost) formats. Users should ensure
% % that all non-photo figures use a vector format (.eps, .pdf, .mps) and
% % not a bitmapped formats (.jpeg, .png). The IEEE frowns on bitmapped formats
% % which can result in "jaggedy"/blurry rendering of lines and letters as
% % well as large increases in file sizes.
% %
% % You can find documentation about the pdfTeX application at:
% % http://www.tug.org/applications/pdftex





% % *** MATH PACKAGES ***
% %
% %\usepackage{amsmath}
% % A popular package from the American Mathematical Society that provides
% % many useful and powerful commands for dealing with mathematics.
% %
% % Note that the amsmath package sets \interdisplaylinepenalty to 10000
% % thus preventing page breaks from occurring within multiline equations. Use:
% %\interdisplaylinepenalty=2500
% % after loading amsmath to restore such page breaks as IEEEtran.cls normally
% % does. amsmath.sty is already installed on most LaTeX systems. The latest
% % version and documentation can be obtained at:
% % http://www.ctan.org/pkg/amsmath





% % *** SPECIALIZED LIST PACKAGES ***
% %
% %\usepackage{algorithmic}
% % algorithmic.sty was written by Peter Williams and Rogerio Brito.
% % This package provides an algorithmic environment fo describing algorithms.
% % You can use the algorithmic environment in-text or within a figure
% % environment to provide for a floating algorithm. Do NOT use the algorithm
% % floating environment provided by algorithm.sty (by the same authors) or
% % algorithm2e.sty (by Christophe Fiorio) as the IEEE does not use dedicated
% % algorithm float types and packages that provide these will not provide
% % correct IEEE style captions. The latest version and documentation of
% % algorithmic.sty can be obtained at:
% % http://www.ctan.org/pkg/algorithms
% % Also of interest may be the (relatively newer and more customizable)
% % algorithmicx.sty package by Szasz Janos:
% % http://www.ctan.org/pkg/algorithmicx




% % *** ALIGNMENT PACKAGES ***
% %
% \usepackage{array}
% \usepackage{booktabs}
% % Frank Mittelbach's and David Carlisle's array.sty patches and improves
% % the standard LaTeX2e array and tabular environments to provide better
% % appearance and additional user controls. As the default LaTeX2e table
% % generation code is lacking to the point of almost being broken with
% % respect to the quality of the end results, all users are strongly
% % advised to use an enhanced (at the very least that provided by array.sty)
% % set of table tools. array.sty is already installed on most systems. The
% % latest version and documentation can be obtained at:
% % http://www.ctan.org/pkg/array


% % IEEEtran contains the IEEEeqnarray family of commands that can be used to
% % generate multiline equations as well as matrices, tables, etc., of high
% % quality.




% % *** SUBFIGURE PACKAGES ***
% % \ifCLASSOPTIONcompsoc
% %  \usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
% % \else
% %  \usepackage[caption=false,font=footnotesize]{subfig}
% % \fi
% % \captionsetup[subfloat]{listofindent=4em,listofformat=parens}
% \usepackage{subfigure}
% % \usepackage{caption}
% %\usepackage{subcaption}
% % subfig.sty, written by Steven Douglas Cochran, is the modern replacement
% % for subfigure.sty, the latter of which is no longer maintained and is
% % incompatible with some LaTeX packages including fixltx2e. However,
% % subfig.sty requires and automatically loads Axel Sommerfeldt's caption.sty
% % which will override IEEEtran.cls' handling of captions and this will result
% % in non-IEEE style figure/table captions. To prevent this problem, be sure
% % and invoke subfig.sty's "caption=false" package option (available since
% % subfig.sty version 1.3, 2005/06/28) as this is will preserve IEEEtran.cls
% % handling of captions.
% % Note that the Computer Society format requires a larger sans serif font
% % than the serif footnote size font used in traditional IEEE formatting
% % and thus the need to invoke different subfig.sty package options depending
% % on whether compsoc mode has been enabled.
% %
% % The latest version and documentation of subfig.sty can be obtained at:
% % http://www.ctan.org/pkg/subfig




% % *** FLOAT PACKAGES ***
% %
% %\usepackage{fixltx2e}
% % fixltx2e, the successor to the earlier fix2col.sty, was written by
% % Frank Mittelbach and David Carlisle. This package corrects a few problems
% % in the LaTeX2e kernel, the most notable of which is that in current
% % LaTeX2e releases, the ordering of single and double column floats is not
% % guaranteed to be preserved. Thus, an unpatched LaTeX2e can allow a
% % single column figure to be placed prior to an earlier double column
% % figure.
% % Be aware that LaTeX2e kernels dated 2015 and later have fixltx2e.sty's
% % corrections already built into the system in which case a warning will
% % be issued if an attempt is made to load fixltx2e.sty as it is no longer
% % needed.
% % The latest version and documentation can be found at:
% % http://www.ctan.org/pkg/fixltx2e


% %\usepackage{stfloats}
% % stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e
% % the ability to do double column floats at the bottom of the page as well
% % as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in
% % LaTeX2e). It also provides a command:
% %\fnbelowfloat
% % to enable the placement of footnotes below bottom floats (the standard
% % LaTeX2e kernel puts them above bottom floats). This is an invasive package
% % which rewrites many portions of the LaTeX2e float routines. It may not work
% % with other packages that modify the LaTeX2e float routines. The latest
% % version and documentation can be obtained at:
% % http://www.ctan.org/pkg/stfloats
% % Do not use the stfloats baselinefloat ability as the IEEE does not allow
% % \baselineskip to stretch. Authors submitting work to the IEEE should note
% % that the IEEE rarely uses double column equations and that authors should try
% % to avoid such use. Do not be tempted to use the cuted.sty or midfloat.sty
% % packages (also by Sigitas Tolusis) as the IEEE does not format its papers in
% % such ways.
% % Do not attempt to use stfloats with fixltx2e as they are incompatible.
% % Instead, use Morten Hogholm'a dblfloatfix which combines the features
% % of both fixltx2e and stfloats:
% %
% % \usepackage{dblfloatfix}
% % The latest version can be found at:
% % http://www.ctan.org/pkg/dblfloatfix




% % *** PDF, URL AND HYPERLINK PACKAGES ***
% %
% %\usepackage{url}
% % url.sty was written by Donald Arseneau. It provides better support for
% % handling and breaking URLs. url.sty is already installed on most LaTeX
% % systems. The latest version and documentation can be obtained at:
% % http://www.ctan.org/pkg/url
% % Basically, \url{my_url_here}.




% % *** Do not adjust lengths that control margins, column widths, etc. ***
% % *** Do not use packages that alter fonts (such as pslatex).         ***
% % There should be no need to do such things with IEEEtran.cls V1.6 and later.
% % (Unless specifically asked to do so by the journal or conference you plan
% % to submit to, of course. )

% %\usepackage[subtle]{savetrees}

% \begin{document}

% \pagestyle{fancy}
% \fancyfoot{}
% \fancyhead{}
% \renewcommand{\headrulewidth}{0pt}
% \fancyfoot[C]{\textbf{Unpublished work. Please do not share.}}
% % \fancyhead[C]{Submitted to DATE 2023}

% %
% % paper title
% % Titles are generally capitalized except for words such as a, an, and, as,
% % at, but, by, for, in, nor, of, on, or, the, to and up, which are usually
% % not capitalized unless they are the first or last word of the title.
% % Linebreaks \\ can be used within to get better formatting as desired.
% % Do not put math or special symbols in the title.
% \title{Chiplets: How Small is too Small?}


% % author names and affiliations
% % use a multiple column layout for up to three different
% % affiliations

% \author{\IEEEauthorblockN{Alexander Graening, Saptadeep Pal, Puneet Gupta}
% \IEEEauthorblockA{Department of Electrical and Computer Engineering\\
% University of California, Los Angeles\\
% agraening@ucla.edu, saptadeep@ucla.edu, puneet@ee.ucla.edu}}


% % conference papers do not typically use \thanks and this command
% % is locked out in conference mode. If really needed, such as for
% % the acknowledgment of grants, issue a \IEEEoverridecommandlockouts
% % after \documentclass




% % use for special paper notices
% %\IEEEspecialpapernotice{(Invited Paper)}




% % make the title area
% \maketitle



% % As a general rule, do not put math, special symbols or citations
% % in the abstract
% \begin{abstract}
% As chiplet systems increase in popularity, it is important to revisit the tradeoffs for converting a monolithic design to a chiplet system. Chip yield, reusability, performance binning, and floorplanning considerations push us toward smaller chiplets. Meanwhile, inter-chiplet interconnect and chiplet assembly overheads push us toward larger chips both in terms of power requirements and cost. This work explores the impacts of these considerations on the {\em minimum} chiplet size that makes sense. We examine the case of a large design that could be built as a single monolithic system on chip (SoC) or as a system of chiplets and show that optimal chiplet size depends on a wide range of parameters. Our analysis indicates that the smallest chiplet sizes that are viable cost-wise are between 40mm$^2$ and 80mm$^2$ for microprocessor type logic and between 150mm$^2$ and 200mm$^2$ for random logic making the case for chipletization weaker for all but the largest SoCs.

% \end{abstract}

% % no keywords




% % For peer review papers, you can put extra information on the cover
% % page as needed:
% % \ifCLASSOPTIONpeerreview
% % \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% % \fi
% %
% % For peerreview papers, this IEEEtran command inserts a page break and
% % creates the second title. It will be ignored for other modes.
% % \IEEEpeerreviewmaketitle



% %%%%%%%%%%%%%%%
% % Readability %
% %%%%%%%%%%%%%%%
% % Note: For readability follow the style below. This makes it easy to locate where you are in the text to edit.
% % - Before each section, add a title in a "comment box" as above.
% % - Before the "comment box" leave 3 lines empty.
% % - Before a subsection, leave 2 lines empty.
% % - Before a subsubsection, leave 1 line empty.
% % - Always skip 1 line after a section, subsection, or subsubsection line.
% % - Always indent the content of a section, subsection, or subsubsection relative to the previous level of hierarchy.



% %%%%%%%%%%%%%%%%%%%%%%%%
% % Introduction Section %
% %%%%%%%%%%%%%%%%%%%%%%%%
% \section{Introduction}
    
%     Chiplet systems have become popular as a way to improve the yield of systems that would otherwise have unacceptably low yield due to their large total area. This trend runs counter to the previous trend of increasing integration by packing more and more into a single monolithic chip.
    
%     For large designs, splitting into smaller chips can have several advantages. Small chips have higher yield than large chips.  Chiplet reuse in the form of including a single chiplet design in multiple systems allows sharing of design, manufacturing, and testing costs across systems.  If a chiplet contains too much functionality, it can become specialized to a specific design, and the opportunities for reuse are reduced~\cite{Pal2020}.
    
%     There are also drawbacks to splitting a design into chiplets. Assembly and packaging for a design that has been partitioned into chiplets are more costly than they are for a monolithic SoC design. In addition to the costs related to the integration substrate (e.g. silicon interposer) and greatly increased assembly time, yield in the assembly and packaging stage suffer due to the increased number of fine-pitch bonds that must be made and number of individual chiplets that must be assembled. Also, the total silicon area would go up in order to accommodate the additional IO cells needed for inter-chiplet communication. This inter-chiplet communication also increases the overall power consumption of the design.
    
%     In this work, we build an analytical framework to answer the question: what is the right chiplet size when the multitude of manufacturing related factors are considered? We consider a case of a design that is small enough to be manufactured as a monolithic SoC, but is large enough to benefit significantly from splitting into chiplets to improve yield.  Our analysis shows that building systems out of tiny chiplets or chiplets smaller than 40mm$^2$ would not be cost optimal unless advancements to the assembly process are made.
%     %with many different types of chips, but since we must assume some values to provide meaningful results, we look at a \hl{range of values for the most sensitive parameters}.
    
%     % Section \ref{sec:RelatedWork} mentions some previous work on this topic and 
    
%     The paper is organized as follows. Section \ref{sec:DesignConsiderations} models the cost benefits/overheads of breaking an SoC into chiplets.  Section \ref{sec:results} discusses a case study of a large system built using chiplets and analyzes the sensitivity of system cost  to various factors such as defect density, assembly cost, IO size etc.  In Section \ref{sec:other}, we discuss the other related factors (which are often architecture dependent and therefore difficult to quantify in general) that would also effect the choice of chiplet size. Finally, Section \ref{sec:conclusion} concludes the work.



% % \hl{Related Work}

% % %%%%%%%%%%%%%%%%%%%%%%%%
% % % Related Work Section %
% % %%%%%%%%%%%%%%%%%%%%%%%%
% % \section{Related Work} \label{sec:RelatedWork}

% %     A number of previous works have addressed parts of this problem \hl{...}
    
% %     The work \cite{Singh1994} discusses an application of Rent's Rule to multi-chip modules considering a figure of merit consisting of a weighted sum of cost, silicon efficiency, and quality. The paper provides a valuable analytical model for evaluating chiplet sizing, but does not address power and performance as considerations for chiplet sizing. Additionally, it does not consider the size of IO cells or assembly costs that scale with number of chiplets.
    
% %     \hl{...}

% %     Our contribution is that we combine \hl{...} factors and add the consideration of \hl{...} to the models.

% %     % We include IO cell area and ESD protection as a factor in the design and consider assembly costs and yield implications of multi-chiplet designs.



% %%%%%%%%%%%%%%%%%%%%%%%%%%
% % Small Chiplets Section %
% %%%%%%%%%%%%%%%%%%%%%%%%%%
% % \section{Why do we Want Small Chiplets?} \label{sec:SmallChiplet}
    


% % Ultimately, this could be similar to how printed circuit board (PCB) designs take several off-the-shelf packaged chips and place them together on the same board. 2.5D integration for chiplet systems may be used similarly if chiplets are designed to be useful across multiple systems. Unfortunately, if a chiplet contains multiple functions for a larger design, this can make it very specific to the system it is designed for and unlikely to be useful in other future designs. As chip complexity scales with size, this means that large chiplets will tend to be more system specific than smaller designs. This gives us incentive to try to make chiplets as small as possible without incurring additional costs.



% %%%%%%%%%%%%%%%%%%%%%%%%%%
% % Design Factors Section %
% %%%%%%%%%%%%%%%%%%%%%%%%%%
% %\section{Important Design Considerations} \label{sec:DesignConsiderations}
% \section{Cost Implications of Chipletization} \label{sec:DesignConsiderations}
%     In this section, we quantify and model some of the most important factors that affect the cost of manufacturing a system using chiplets.
    
%     %we discuss a few of these that are easy to quantify and start to build a model for analyzing design cost based on chiplet size.
%     % Chiplet systems place additional constraints on floorplanning and on interconnections between chiplets that must be taken into account during the design phase.\hl{edit}
    
%     % \subsection{Top Level Wirelength Overhead}
    
%     %     Wire length increases as the design is split into more and more chiplets. This increase in wire length is due to the minimum distance of separation between chiplets. 
        
%     %     \hl{Add a figure showing how communication overhead scales with chiplet size.}


%     \subsection{IO Cells}
        
%         Splitting a design into chiplets introduces the requirement for inter-chiplet communication. This adds overhead in terms of area and power requirements for interconnect wires and IO cells to provide ESD protection and drive relatively long connections between chiplets \cite{Pal2020pathfinding}.
        
%         \subsubsection{ESD Requirements}

%             The amount of ESD protection necessary for 2.5D designs is not a settled question, but there is some consensus that the ``external'' IO cells that will be connected to external pins on the finished module will need higher levels of protection than ``internal'' IO cells that will not be connected to external pins, drive only inter-chiplet wires and will only be exposed to ESD in the manufacturing process. For external IO cells, JEDEC recommendations suggest meeting 250V Charged Device Model (CDM) protection  \cite{JEDEC-CDMrec2022}. On the other hand, a TSMC discussion of a Lite-IO cell design for inter-chiplet communication only uses 10V CDM protection \cite{Cheng2020}. Whether ESD protection is necessary and how much is necessary for inter-chiplet connections depends on process specifications, so we look at a range of levels of protection from 0V to 500V CDM.
            
%             % 500V Human Body Model (HBM) protection (although 1kV and 2kV HBM are common) \cite{JEDEC-HBMrec2018} and 
            
%         \subsubsection{Area Impact of ESD}
        
%             Due to ESD protection, the total design area will increase due to the IO cell area for inter-chiplet connections in addition to the overhead due to minimum separation distance between chiplets. In order to determine the IO cell size necessary to meet different levels of ESD protection, we ran SPICE simulations using the circuit shown in Figure \ref{fig:spice_sim_sch}. The clamp is assumed to be shared among many IO cells, so this is not included in IO cell area calculations.
            
%             % \hl{Insert figure with schematic and box around IO cell portion of the circuit.}
            
%             By setting different initial voltages for the capacitor in the above model, we tested different levels of CDM protection. For the purposes of this study, the device was considered to pass if the voltage never passed the voltage breakdown level of the gate oxide. Other types of incremental damage can also occur as a result of ESD events \cite{Amerasekera1992}, but were not considered here as we wanted a simple metric of pass or fail. Buffer sizes were taken from \cite{Pal2021}.
            
%             % \hl{Add note on commercial IO cell sizes and Saptadeep's IO cells for 2.5D system.}
            
%             % \begin{figure}[t!]
%             %     \centering
%             %     \includegraphics[width=3.5in]{io_cell_sizes_esd.png}
%             %     \caption{Area requirements for RX IO Cells. Note that for TX cells, ESD protection is not always necessary since the pad is not connected to the MOSFET gate \cite{Cheng2020}.}
%             %     \label{fig:io_cell_sizes_esd}
%             % \end{figure}
            
%             \begin{table}[htbp]
%                 \centering
%                 \caption{Area requirements for IO cells by ESD protection level in 40nm. Note that these IO cell sizes are for simple IO cells designed for inter-chiplet connections. External IOs would use much larger IO cells, e.g. GPIO cells in 28nm of 3,250$\mu$m$^2$ \cite{certus28nm} and in 12nm that are 1,500$\mu$m$^2$ \cite{certus12nm} are routinely used in products.}
%                 \begin{tabular}{|c|c|c|c|c|c|}
%                     \cmidrule{3-5}    \multicolumn{1}{r}{} &       & \multicolumn{3}{c|}{Area (${\mu}m^2$)} &                        \multicolumn{1}{r}{} \\
%                     \midrule
%                     ESD(V) & Diode Pairs & ESD   & Buffer & IO Cell & ESD Cap(fF) \\
%                     \midrule
%                     0     & 0     & 0.00  & 47.63 & 47.63 & 0.00 \\
%                     \midrule    
%                     10    & 2     & 15.02 & 47.63 & 62.65 & 8.02 \\
%                     \midrule
%                     125   & 6     & 45.07 & 47.63 & 92.70 & 18.97 \\
%                     \midrule
%                     250   & 11    & 82.62 & 47.63 & 130.25 & 37.65 \\
%                     \midrule
%                     500   & 20    & 150.22 & 47.63 & 197.85 & 74.97 \\
%                     \bottomrule
%                 \end{tabular}%
%                 \label{tab:io_cell_sizes_esd}%
%             \end{table}%
            
%             As a design is partitioned into more and more chiplets, the area requirement for IO cells increases substantially since the increasing number of inter-chiplet interconnects need ESD protection and larger driver circuits.
            
%             \begin{figure}[t]
%                 \centering
%                 \includegraphics[width=3.0in]{spice_sim_sch.png}
%                 \caption{ESD Simulation Structure. The number of diode pairs connected $V_{PAD}$ are swept to find the number necessary to keep $V_{IO}$ below the breakdown voltage of the gate dielectric. The ESD event model is from \cite{Baker2019}.}
%                 \label{fig:spice_sim_sch}
%             \end{figure}
            
            
%             % \setcounter{lofdepth}{3}
%             % \listoffigures \medskip
            
%             % \begin{figure*}[t!]
%             %     \centering
%             %     \includegraphics[width=7.1in]{CombinedAreaCostPowerPlots.png}
%             %     \caption{(a) Percentage of Area Consumed by IO Cells for Different IO Densities Ranging from 100 IOs/mm$^2$ to 2000 IOs/mm$^2$. (b) Power Wasted by IO Cells for Different IO Densities Ranging from 100 IOs/mm$^2$ to 2000 IOs/mm$^2$. (c) Cost per mm$^2$ for different chiplet size and defect densities. This assumes square chiplets fit into a 26x33mm reticle.}
%             %     \label{fig:combined_area_cost_power}
%             % \end{figure*}
            
%             % \begin{figure}
%             %     \centering
%             %     \includegraphics[width=2.5in]{WastedAreaIO_Density.png}
%             %     \caption{Percentage of Area Consumed by IO Cells for Different IO Densities Ranging from 100 IOs/mm$^2$ to 2000 IOs/mm$^2$.}
%             %     \label{fig:WastedAreaIO_Density}
%             % \end{figure}
            
%             % \begin{figure}
%             %     \centering
%             %     \includegraphics[width=2.5in]{IOCellPower.png}
%             %     \caption{Extra Energy per Bit for Inter-Chiplet Communication for Different IO Densities Ranging from 100 IOs/mm$^2$ to 2000 IOs/mm$^2$.}
%             %     \label{fig:IOCellPower}
%             % \end{figure}
            
%             \begin{figure}
%                 \centering
%                 \includegraphics[width=3.4in]{WastedAreaIO_Density__IOCellPower.png}
%                 \caption{Left: Extra Energy per Bit for Inter-Chiplet Communication for Different IO Densities. Right: Percentage of Area Consumed by IO Cells for Different IO Densities. Both: IO densities range from 100 IOs/mm$^2$ to 2000 IOs/mm$^2$}
%                 \label{fig:WastedAreaIO_Density__IOCellPower}
%             \end{figure}
            
%             % \begin{figure*}[ht]
%             %     \centering
%             %     \begin{subfigure}
%             %         \centering
%             %         \includegraphics[width=2.2in]{WastedAreaIO_Density.png}
%             %         \caption{Percentage of Area Consumed by IO Cells for Different IO Densities Ranging from 100 IOs/$mm^2$ to 2000 IOs/$mm^2$.}
%             %         \label{fig:WastedAreaIO_Density}
%             %     \end{subfigure}
%             %     \hfill
%             %     \begin{subfigure}
%             %         \centering
%             %         \includegraphics[width=2.2in]{IOCellPower.png}
%             %         \caption{Power Wasted by IO Cells for Different IO Densities Ranging from 100 IOs/$mm^2$ to 2000 IOs/$mm^2$.}
%             %         \label{fig:IOCellPower}
%             %     \end{subfigure}
%             %     \hfill
%             %     \begin{subfigure}
%             %         \centering
%             %         \includegraphics[width=2.2in]{reticle_fit.png}
%             %         \caption{The three examples above (left to right): an example of large chiplet designs that fit evenly into the reticle size, an example of large chiplets that fit poorly into the reticle size, and an example of a poorly fitting small chiplet. Overhead for a bad fit is lower for small chiplets.}
%             %         \label{fig:reticle_fit}
%             %     \end{subfigure}
%             %     \caption{Need to fix this figure}
%             %     \label{}
%             % \end{figure*}
            
%             To compute the impact of IO cells on area,  IO densities are scanned from 100-2000 IOs/mm$^2$ across multiple levels of ESD protection. Results are shown in Figure \ref{fig:WastedAreaIO_Density__IOCellPower}.
            
%             Inter-chiplet IOs also cost extra energy in order to drive the inter-chiplet interconnect wire and the additional capacitance added by the ESD diodes. To compute energy per bit, we used wire parasitics from a commercial 40nm PDK and the ESD diode capacitance. The interconnect wirelength was estimated from the inter-die separation (assumed to be 300$\mu$m) and area of the IO cells assuming multiple rows of boundary placed IO cells, similar to the methodology in~\cite{Pal2020pathfinding}. The cost in energy per bit is shown in Figure \ref{fig:WastedAreaIO_Density__IOCellPower}.
            

        
%             % \begin{figure}[t!]
%             %     \centering
%             %     \includegraphics[width=3.2in]{IOCostMillimeter.png}
%             %     \caption{IO Area Cost Per $mm^2$ for Different IO Densities Ranging from 100 IOs/$mm^2$ to 2000 IOs/$mm^2$.}
%             %     \label{fig:IOCostMillimeter}
%             % \end{figure}
            
%             % \hl{Ideally, we should have a better area approximation than the 4x diode size approximation we have been using.}
            
%             % \hl{Also, the driver size estimate should be more reliable than a guess based on Saptadeep's layout image in his IO cell paper.}



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Manufacturing Factors Section %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \section{Important Manufacturing Considerations} \label{sec:ManufacturingConsiderations}
%     % In the manufacturing stage, we need to consider factors that contribute to the cost of the system such as silicon cost, cost of assembly, and yield. \hl{edit}


%     \subsection{Chiplet Cost}
    
%         Individual chiplet cost is dependent on the individual chiplet yield. Taking $k_{die}$ as the cost per untested die, the actual cost per die is given by Equation \ref{eq:dieCost}.
        
%         \begin{equation} \label{eq:dieCost}
%             C_{die} = \frac{k_{die}}{Y_{die}}
%         \end{equation}
        
%         The cost per untested die ($k_{die}$) is dependent both on the area of the die and on how well the die fits into the reticle size. The impact of utilization of the reticle size is negligible for small chiplets, but can have a larger effect for chiplets that are relatively large compared to the reticle. This cost is the result of needing an increased number of lithographic exposures to manufacture dies that do not evenly divide into the reticle field \cite{Jeong2011}.  The cost per untested die is given below in Equation \ref{eq:costReticle}.
        
%         % \hl{Note that we are only looking at square chiplets since Rent's Rule does not hold true if we change the aspect ratio of the dies} \cite{Stroobandt2001}. \hl{Rent's Rule is used to calculate IO density in the example study.}
        
%         \begin{equation} \label{eq:costReticle}
%             k_{die} = k_{silicon}chip\_area+\frac{k_{exposures}}{\left\lfloor \frac{reticle\_area}{chip\_area} \right\rfloor}
%         \end{equation}
        
%         Where $k_{silicon}$ is the cost per unit area,  and $k_{exposures}$ is the cost per exposure. We assume the lithography cost is 34\% of the total wafer cost \cite{Patel2018}.
        
%         % The cost per exposure given in \cite{Jeong2011} for 45nm is estimated as \$0.69, \$2.07, or \$3.45 depending on the criticality of the layer in question.
        
%         Die yield can be given by Equation \ref{eq:y_die}. This yield model is taken from \cite{Kuo1999}, but split into two components: die yield and assembly yield.
        
%         \begin{equation} \label{eq:y_die}
%             Y_{die}=Y_{wp}\left( 1 + \frac{A_cD_0}{\alpha} \right) ^{-\alpha}
%         \end{equation}
        
%         Where $Y_{wp}$ is the wafer process yield assumed to be 94\% \cite{Kuo1999}.  $A_c$ is the critical area. For the purposes of this study, we use the core area (excluding IO area) as critical area. For a more accurate analysis of a real design, the actual critical area of the design should be computed and used here instead of the core area. $D_0$ is the defect density. We use a value of 0.004/mm$^2$ from \cite{chen2010} and also look at defect densities of 0.008/mm$^2$ and 0.002/mm$^2$. $\alpha$ is the clustering factor for defects and we use a value of 2 \cite{chen2010}.

%         \begin{figure}
%             \centering
%             \includegraphics[width=2.8in]{reticle_fit.png}
%             \caption{Reticle Fit Cost. The three examples above (left to right): an example of a large chiplet design that fits evenly into the reticle size; an example of large chiplets that fit poorly into the reticle size; and an example of a poorly fitting small chiplet. Overhead for a bad fit is lower for small chiplets.}
%             \label{fig:reticle_fit}
%         \end{figure}
            
%         \begin{figure}
%             \centering
%             \includegraphics[width=3.0in]{CostPerMMYieldExposure.png}
%             \caption{Silicon Cost for Different Chiplet Sizes and Defect Densities.}
%             \label{fig:CostPerMMYieldExposure}
%         \end{figure}
        
%         In Figure \ref{fig:CostPerMMYieldExposure}, one can see that the cost per mm$^2$ has somewhat of a stepwise behavior depending on how well the chip fits in the reticle size. For this plot, we did not make any assumptions about the aspect ratio of the chips and just considered how well the chip size divides into the reticle. The general trend is due to yield decreasing as chip size increases and the steps are due to the chip size increasing above a number that divides evenly into the 858mm$^2$ (26x33mm) reticle.


%     \subsection{Assembly Cost}
    
%         Assembly time and cost will increase with the number of chiplets. How this scales is dependent on the bonding process. There are two main models we will look at here. In one case, the chips are placed and bonded individually (e.g. in the case of copper pillar thermal compression bonding) giving an assembly time as follows.
        
%         \begin{equation} \label{eq:t_assembly}
%             T_{assembly} = N(T_{place}+T_{bonding})
%         \end{equation}
        
%         On the other hand, it is possible that multiple chips will be placed and tacked individually on the interconnect substrate, but finally bonded at the same time as is the case for solder reflow.
        
%         \begin{equation} \label{eq:t_assembly_simultaneous}
%             T_{assembly} = NT_{place} + T_{bonding}
%         \end{equation}
        
%         % \begin{figure}[t!]
%         %     \centering
%         %     \includegraphics[width=3.2in]{assembly_time.png}
%         %     \caption{Assembly time in seconds compared to number of chiplets. Baseline time for the SoC is 30 seconds with 10 seconds for pick and place and 20 for bonding.}
%         %     \label{fig:assembly_time}
%         % \end{figure}
        
%         In the second case, bonding scales significantly better than in the first case, but the time for pick and place still scales with the number of chips. Interposer cost is discussed in \cite{Li2013}. The cost of assembly can be modeled by looking at materials cost and machine operating cost as shown below.
        
%         \begin{equation} \label{eq:c_assembly}
%             C_{assembly}=C_{interposer}+k_{machine}T_{assembly}
%         \end{equation}
        
%         The machine operating cost of assembly for the machine or machines used consists of the amortized cost of the equipment and maintenance over the equipment lifetime plus the cost of electricity and technician salaries. To compute values for $k_{machine}$, we assume machine costs of \$200k-\$2M depreciated over 5 years with full-time personnel costs of \$200k per year and 90\% uptime with a single bonding head.
        
%         Bonding time for Cu-Cu pillar bonding is 20 seconds \cite{Bajwa2017} and hybrid bonding is shorter at 10 seconds \cite{Ohyama2015}. Since hybrid bonding and Cu-Cu pillar bonding offer low pitch interconnects (down to 10um \cite{Lau2022}\cite{Bajwa2017}), we do not consider other types of bonding for this study. Pick and place time is assumed to be somewhere from 2-10 seconds per die. In Figure \ref{fig:assembly_cost}, we assume Cu-Cu pillar bonding and 10 seconds for pick and place, but the trend holds for other types of bonding as well. The interposer cost is taken from \cite{Li2013}.
%         % This is shown in equation \ref{eq:k_machine}.
        
%         % \begin{equation} \label{eq:k_machine}
%         %     k_{machine}=\frac{C_{machine}+C_{maintenance}}{T_{lifetime}}+k_{operation}
%         % \end{equation}
        
%         The values for assembly time and machine costs vary linearly with respect to the number of chiplets. Assembly yield is another consideration for the cost of assembly. The assembly yield scales with the number of interconnects and the number of chiplets.
        
%         \begin{equation} \label{eq:y_assembly}
%             Y_{assembly} = (N_{die}Y_{alignment})\times(N_{pins}Y_{pins})
%         \end{equation}

%         In Equation \ref{eq:y_assembly}, the first term is the yield of die alignment and the second is the pin bonding yield. The more dies there are in the multi-chiplet system, the higher the risk of misalignment and the more pins that need to be bonded, the higher the risk that a pin will not bond correctly. Since we are not making assumptions about IO density yet, Figure \ref{fig:assembly_cost} does not include yield although we include assembly yield in our analysis in the next section. We assume values of 99.9\% for $Y_{alignment}$ and 99.9999\% for $Y_{bonding}$ \cite{Gao2019}.

%         \begin{figure}[t!]
%             \centering
%             \includegraphics[width=3.2in]{assembly_cost.png}
%             \caption{Assembly Machine and Personnel Cost by Number of Chiplets. IB stands for individual bonding, SB stands for simultaneous bonding, M1 refers to \$200,000 machine, M2 refers to \$1,000,000 machine, and M3 refers to \$2,000,000 machine. FP stands for 2-second pick and place, SP indicates 10 seconds. This plot uses Cu-Cu pillar bonding time (20 seconds) in all cases.}
%             \label{fig:assembly_cost}
%         \end{figure}



% %%%%%%%%%%%%%%%%%%%
% % Results Section %
% %%%%%%%%%%%%%%%%%%%
% \section{Results} \label{sec:results}

%     % Add discussion of real case and comparison to Rent's Rule analysis. \hl{This could likely be a 1400 core version of Saptadeep's design.}

%     In this section, we discuss the results of applying the above analysis to an example case where we take an 800mm$^2$ chip and split it into evenly sized chiplets.
    
%     The cost may be found using Equation \ref{eq:CostFOM}.
        
%     \begin{equation} \label{eq:CostFOM}
%         C = \frac{1}{Y_{assembly}} \left[ \left( \sum_{i=1}^{N_c} C_{die} \right) + C_{assembly}    \right]
%         % C = \frac{1}{Y} \left[ \left( \sum_{i=1}^{N_c} C_{die} \right) + n_{l}C_{l} + C_{test} + C_{asm}    \right]
%         % C = \frac{1}{Y} \left[ \left( \sum_{i=1}^{N_c} C_{die} \right) + \left( n_{l}C_{l}+C_{int} \right) + C_{t} + C_{asm}    \right]
%         % C_{mcm} = \frac{1}{Y_{mcm}} \left[ \left( \sum_{i=1}^{N_c} C_{die} \right) + \left( n_{layers}C_{layer}+C_{interposer} \right) + C_{test} + C_{assembly} \right]
%     \end{equation}
    
%     Where $C$ is the total cost and both $Y_{assembly}$ and $C_{die}$ are given in the previous sections. There is one more piece we need to be able to apply this analysis and that is the number of IOs per chiplet. To do this, we use Rent's Rule as shown in Equation \ref{eq:Rent'sRule} \cite{Stroobandt2000}.
    
%     \begin{equation} \label{eq:Rent'sRule}
%         N_p = kN_g^a
%     \end{equation}
    
%     Here $N_p$ is the number of pins or IOs, $N_g$ is the number of gates in the design, and k and a are constants that depend on the architecture. Rent's Rule gives us a way of estimating how the number of IOs scales with different sized chips assuming the chips are the same types of design. Although the Rent's Rule constants are design specific, this allows us to draw some useful conclusions.
    
%     To estimate the number of gates in the design we divided the area by the size of an AND gate in 40nm. We use two sets of constants, the primary set of constants we used is given in \cite{Singh1994} as values of the constants for a microprocessor architecture and we compare to the values given in the same paper for random logic in the comparison for levels of ESD protection below.
    
%     Unless otherwise stated, the following plots us medium defect density (0.004/mm$^2$), 125V CDM ESD protection, microprocessor Rent's Rule constants, and M2 (\$1M machine) with 30 second individual bonding of chiplets in accordance with Equation \ref{eq:t_assembly}.
    
%     % Where $C$ is the total cost, $Y$ is the assembly yield of the completed module, $n_l$ is the number of layers on the interposer, $C_l$ is the cost per layer on the interposer, $C_{int}$ is the area dependent cost of the silicon or other material interposer, $C_t$ is the testing cost, and $C_{asm}$ is the assembly cost. The number of layers $n_l$ can be calculated as shown in equation \ref{eq:nlayers}. \cite{Singh1994}
        
%     % \begin{equation} \label{eq:nlayers}
%     %     n_l = \frac{I_{length} e_{mcm} p_{mcm}}{substrate_{area}}
%     % \end{equation}
        
%     % In equation \ref{eq:nlayers}, $e_{mcm}$ is the wiring efficiency, $p_{mcm}$ is the wiring pitch, $I_{length}$ is the total wire length estimate based on the Rent's Rule analysis.
            
%     % Rent's Rule for the number of pins for a design with a specific area is given by the following equation.
        
%     \subsection{Dependence on Defect Density}
    
%         Defect density affects the rate at which yield decreases when chip size increases. In Figure \ref{fig:CostOfAssembledSystem}, it can be seen that there is a relatively smooth trend in cost for each defect density level and that the chiplet size that minimizes cost is between 40 and 100mm$^2$. Note that for the low defect density, large chiplets only result in a moderate cost increase over the optimal point. In all cases, the assembly cost begins to dominate for very small (and therefor numerous) chiplets. {\em Improving die yield allows manufacturing of both larger monolithic designs and larger chiplets. Conversely, low yield technologies can justify smaller chiplet.}
    
%         \begin{figure}
%             \centering
%             \includegraphics[width=3.3in]{CostOfAssembledSystemInset2.png}
%             % \includegraphics[width=3.4in]{CostOfAssembledSystemInset.png}
%             % \includegraphics[width=3.3in]{CostOfAssembledSystemZoom.png}
%             % \includegraphics[width=3.3in]{CostOfAssembledSystem.png}
%             \caption{Cost for Different Defect Densities. High defect density is 0.008/mm$^2$, medium defect density is 0.004/mm$^2$, and low defect density is 0.002/mm$^2$.}
%             \label{fig:CostOfAssembledSystem}
%         \end{figure}
        
%     \subsection{Dependence on Assembly Cost}
        
%         Assembly cost has a substantial impact on the small, numerous chiplet side of this study. To examine the impact on minimum chiplet size, we held ESD and defect density constant and changed the machine cost and bonding time. We used high defect density M1 and M3 refer to the same \$200k and \$2M machines described earlier. Individual bonding was assumed for this analysis, but the combined time required for the pick and place and bonding ranges from 10 seconds to 30 seconds. In this plot, the minimum cost values range between chiplet size of 40mm$^2$ and 50mm$^2$. The trend seen in Figure \ref{fig:CostOfAssembledSystemBondingTime2Machines} is that {\em faster and cheaper bonding allows for a larger number of smaller chiplets}.
    
%         \begin{figure}
%             \centering
%             \includegraphics[width=3.3in]{CostOfAssembledSystemBondingTime2MachinesInset.png}
%             % \includegraphics[width=3.2in]{CostOfAssembledSystemBondingTime2MachinesZoom.png}
%             % \includegraphics[width=3.2in]{CostOfAssembledSystemBondingTime2Machines.png}
%             \caption{Costs for Different Bonding/Pick and Place Times and Machines. M3 is a \$2,000,000 machine and M1 is a \$200,000 machine.}
%             \label{fig:CostOfAssembledSystemBondingTime2Machines}
%         \end{figure}

%     \subsection{Dependence on IO Size and IO Density} \label{sec:DependenceOnIOSize}
        
%         The cost of IO cells can substantially affect the optimal point for chiplet size and the overall system cost. This necessarily is dependent on level of ESD protection and the IO density. In Figure \ref{fig:CostOfAssembledSystemIO}, we look at different levels of ESD protection for two different sets of Rent's Rule constants: one for microprocessor logic and one for random logic. For the first set of Rent's Rule constants, the difference between different levels of ESD protection is negligible, but for the second set of Rent's Rule constants, the higher IO density means ESD and assembly yield has a larger impact. {\em Inter-chiplet interconnect increases area requirements and lowers assembly yield, so good chiplet designs should prioritize splitting at logical boundaries that minimize inter-chiplet IO.}
        
%         \begin{figure}
%             \centering
%             \includegraphics[width=3.2in]{CostOfAssembledSystemIO.png}
%             \caption{Cost for Different Levels of ESD Protection and Rent's Rule Constants. M refers to the Rent's Rule constants for microprocessor circuits, and RL refers to Rent's rule constants for random logic \cite{Singh1994}.}
%             \label{fig:CostOfAssembledSystemIO}
%         \end{figure}


%     \subsection{Inter-chiplet Communication Power}
    
%         Increased power consumption is an additional cost of chipletization that does not neatly fit into the cost metric described above. Figure \ref{fig:BandwidthPower} shows the additional power consumed due to the capacitance added at chiplet boundaries in the form of ESD protection and top level wires. As can be seen, {\em for highly connected designs (the random logic case), small chiplets ($<$100mm$^2$) may be energy-wise unaffordable.} Harsher ESD requirements exacerbate the problem.  Good chiplet partitioning approaches which minimize inter-chiplet connectivity can help alleviate the energy overheads.
        
%         \begin{figure}
%             \centering
%             % \includegraphics[width=3.2in]{BandwidthPowerInset.png}
%             \includegraphics[width=3.4in]{BandwidthPower.png}
%             \caption{The Additional Power Consumed by Added Wire and ESD Capacitance. Since this measures additional power due to inter-chiplet interconnect, at chiplet size of 800, there are no internal wires and additional power is 0. The plot starts at chiplet size of 10mm$^2$. M stands for microprocessor and RL for random logic Rent's Rule constants. We analyze two cases of inter-chiplet communication intensity: 100Mbps per link and 1Gbps per link. For 4GHz inter-chiplet communication link, 1GBps amounts to a link activity factor of 25\%.}
%             \label{fig:BandwidthPower}
%         \end{figure}



% % %%%%%%%%%%%%%%%%%%%%%%%
% % % Rent's Rule Section %
% % %%%%%%%%%%%%%%%%%%%%%%%
% % \section{Rent's Rule Analysis}


% %     \subsection{Wire Length}

% %         We can use Rent's Rule to estimate the number of IOs for each chiplet and the total wirelength added to the design by splitting the design into chiplets. One important drawback with this analysis is that Rent's Rule is only valid for square chiplets.
        

%     % \subsection{Figures of Merit}
    
%     %     We consider two figures of merit: cost and power. We assume that necessary pipelining and register stages will be added to longer inter-chiplet connections to maintain freqency of operation same as that of the monolithic SoC design. By keeping the frequency of operation the same, we can consider the impact of voltage scaling on power to be representative of performance variation so the metric will be wrapped up in the power metric.
        

        
%             % The average wire length is given by this equation.
        
%             % \hl{Add equations}
        
%             % The gate dimension is given by the following.
        
%             % \begin{equation} \label{eq:gateDimension}
%             %     d_g=\frac{f_g\bar{R}p_w}{e_wn_w}
%             % \end{equation}

%         % \subsubsection{Power}

%         %     The power may be found using equation \ref{eq:powerFOM}.
        
%         %     \begin{equation} \label{eq:powerFOM}
%         %         P_{mcm}=P_{soc}+f_{mcm}\alpha_{mcm}\frac{C_{total}}{2}V_{DD}^2+P_{IO-Leakage}
%         %     \end{equation}
        
%         %     In equation \ref{eq:powerFOM}, $C_{total}$ is the total capacitance of the top level interconnect wires between chiplets, $\alpha_{mcm}$ is the activitiy factor, $P_{soc}$ is the power of the monolithic design, $V_{DD}$ is the power supply voltage, $f_{mcm}$ is the frequency of operation, and $P_{IO-Leakage}$ is the leakage power due to the IO cells. For the purposes of this study, we are assuming that $f_{mcm} = f_{soc}$ and that $P_{IO-Leakage}$ is negligible.



% %%%%%%%%%%%%%%%%%%%%%%%%%
% % Other Factors Section %
% %%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Other Chiplet Size Tradeoffs} \label{sec:other}


%     \subsection{Floorplanning Overhead}
    
%         In a design consisting solely of ``hard'' IP blocks (blocks with a fixed layout), there may be some wasted area after packing the IP blocks into a rectangular chip. If we consider SoC floorplanning as a rectangle packing problem~\cite{huang2013}, packing all these IP blocks into a single monolithic design will result in less wasted area than packing the IP blocks into several smaller chiplets that each containing fewer IP blocks. 
%         %Although the exact amount of wasted space depends on the shapes of the IP blocks, in \cite{huang2013}, the optimal solutions for rectangle packing shows that a smaller chip with a subset of IPs would result in more wasted space than a bigger monolithic chip. 
%         %Larger numbers of rectangles tend to result in a smaller percentage of space wasted. 
%         For reference, the optimal solutions to the Consecutive Squares benchmark for 2-10 squares contain between 2.86\% and 16.7\% empty space while the optimal solutions for more than 20 blocks all contain less than 1\% empty area. This indicates that the packing problem will result in more inefficiency for smaller chiplet sizes when using ``hard'' IP blocks.
        
%         This effect is less pronounced when using ``soft'' IP blocks or a mix of ``soft'' and ``hard'' IP blocks, since this allows more flexibility in floorplanning and more efficient packing of IP blocks. This case still benefits from larger groups of IPs since smaller groups will increase the likelihood of chiplets with significantly different sizes that can be difficult to fit together efficiently without wasted area on the interposer.
        
%         Since this effect is difficult to quantify for real designs we did not directly consider it in the above analysis. It is important to keep in mind however that wasted area is minimized by including everything in a single SoC as this gives the greatest flexibility of floorplanning and eliminates minimum chiplet separation distances.
    

%     \subsection{Test Cost}
    
%         The testing process is impacted by splitting a monolithic design into multiple chiplets. On one hand, smaller chips provide the opportunity for more fine-grained tests. This can improve the quality of the final product \cite{Singh1994}. Although the chips will be better tested, testing time goes up since chips will be tested individually before being assembled on the interposer and likely again after assembly to ensure assembly did not introduce any errors.


%     \subsection{Non-Recurring Engineering Cost}
        
%         Non-Recurring Engineering (NRE) costs include costs such as masks and tooling that occur regardless of manufacturing volume. In this analysis, we have assumed a high manufacturing volume so these costs can be small. For low volume manufacturing, NRE costs can become a significant factor making smaller chiplets less cost-effective (due to a greater number of masks). 


%     \subsection{Reuse of Chiplets}
    
%         As discussed in \cite{Iyer2019} and \cite{Pal2020}, chiplet reuse scales with the size of chiplets and is impacted by the type of chiplets. A heterogeneous chiplet system can be well-suited to chiplet IP reuse across separate designs. Ultimately, the development time and cost of future designs can be reduced if chiplets are thoughtfully designed as functional blocks that are useful across many systems. Predicting and modeling reuse patterns is difficult and is out of scope for this work.


%     \subsection{Delay-Aware Chiplet Yield}
        
%         % Yield and power (large homogeneous many-core system such as AMD ryzen)
        
%         In many-core homogenous systems, the entire system must run faster than a certain minimum frequency or be considered defective. This means that for a monolithic system, the entire chip will be considered defective if a single core falls below this threshold.  Testing chiplets and only using known good dies in the assembly improves yield.  Yield can drop off quickly for chiplets containing many cores depending on the maximum delay distribution as shown in Figure \ref{fig:DelayVariationYield}. This study comes with several caveats as performance binning, adaptive voltage scaling, multiple clock domains, etc. all can help mitigate this performance-limited yield issue (albeit with other power or cost overheads). Here, we assume a Gaussian distribution of maximum delay \cite{Sartori2010}.
        
%         % Binning chiplets allows taking advantage of process variation to group chiplets with similar performance together so high performing chiplets are not held back by slower chiplets. This will improve frequency of operation on average.
        
%         \begin{figure}
%             \centering
%             \includegraphics[width=3.4in]{DelayVariationYield.png}
%             \caption{Yield with Number of Cores Per Chiplet. The delay distribution for cores is assumed to be Gaussian with a mean of 1000ps and sigma as marked in the legend. This plot considers delay values above the threshold to fail.}
%             \label{fig:DelayVariationYield}
%         \end{figure}
        
%         Figure \ref{fig:CostOfAssembledSystemPerformanceYield} shows a similar plot to those shown in Section \ref{sec:results}. The default parameters are the same as described in that section, but the performance yield is added in. Note that this assumes a homogeneous many-core system that contains 1mm$^2$ cores, so an 800mm$^2$ chip contains 800 cores. If this is split into 4 chiplets, each 200mm$^2$ chiplet contains 200 cores.
        
%         \begin{figure}
%             \centering
%             \includegraphics[width=3.4in]{CostOfAssembledSystemPerformanceYield.png}
%             \caption{Cost of Assembled System with Performance-Aware Yield.}
%             \label{fig:CostOfAssembledSystemPerformanceYield}
%         \end{figure}

%         % \hl{Add analysis of how model in binning paper will affect operating voltage and power consumption assuming there is not a sophisticated method of tuning power supply for each core.}


% % An example of a floating figure using the graphicx package.
% % Note that \label must occur AFTER (or within) \caption.
% % For figures, \caption should occur after the \includegraphics.
% % Note that IEEEtran v1.7 and later has special internal code that
% % is designed to preserve the operation of \label within \caption
% % even when the captionsoff option is in effect. However, because
% % of issues like this, it may be the safest practice to put all your
% % \label just after \caption rather than within \caption{}.
% %
% % Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% % option should be used if it is desired that the figures are to be
% % displayed while in draft mode.
% %
% %\begin{figure}[!t]
% %\centering
% %\includegraphics[width=2.5in]{myfigure}
% % where an .eps filename suffix will be assumed under latex, 
% % and a .pdf suffix will be assumed for pdflatex; or what has been declared
% % via \DeclareGraphicsExtensions.
% %\caption{Simulation results for the network.}
% %\label{fig_sim}
% %\end{figure}

% % Note that the IEEE typically puts floats only at the top, even when this
% % results in a large percentage of a column being occupied by floats.


% % An example of a double column floating figure using two subfigures.
% % (The subfig.sty package must be loaded for this to work.)
% % The subfigure \label commands are set within each subfloat command,
% % and the \label for the overall figure must come after \caption.
% % \hfil is used as a separator to get equal spacing.
% % Watch out that the combined width of all the subfigures on a 
% % line do not exceed the text width or a line break will occur.
% %
% %\begin{figure*}[!t]
% %\centering
% %\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
% %\label{fig_first_case}}
% %\hfil
% %\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
% %\label{fig_second_case}}
% %\caption{Simulation results for the network.}
% %\label{fig_sim}
% %\end{figure*}
% %
% % Note that often IEEE papers with subfigures do not employ subfigure
% % captions (using the optional argument to \subfloat[]), but instead will
% % reference/describe all of them (a), (b), etc., within the main caption.
% % Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% % labels, the optional argument to \subfloat must be present. If a
% % subcaption is not desired, just leave its contents blank,
% % e.g., \subfloat[].


% % An example of a floating table. Note that, for IEEE style tables, the
% % \caption command should come BEFORE the table and, given that table
% % captions serve much like titles, are usually capitalized except for words
% % such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% % and up, which are usually not capitalized unless they are the first or
% % last word of the caption. Table text will default to \footnotesize as
% % the IEEE normally uses this smaller font for tables.
% % The \label must come after \caption as always.
% %
% %\begin{table}[!t]
% %% increase table row spacing, adjust to taste
% %\renewcommand{\arraystretch}{1.3}
% % if using array.sty, it might be a good idea to tweak the value of
% % \extrarowheight as needed to properly center the text within the cells
% %\caption{An Example of a Table}
% %\label{table_example}
% %\centering
% %% Some packages, such as MDW tools, offer better commands for making tables
% %% than the plain LaTeX2e tabular which is used here.
% %\begin{tabular}{|c||c|}
% %\hline
% %One & Two\\
% %\hline
% %Three & Four\\
% %\hline
% %\end{tabular}
% %\end{table}


% % Note that the IEEE does not put floats in the very first column
% % - or typically anywhere on the first page for that matter. Also,
% % in-text middle ("here") positioning is typically not used, but it
% % is allowed and encouraged for Computer Society conferences (but
% % not Computer Society journals). Most IEEE journals/conferences use
% % top floats exclusively. 
% % Note that, LaTeX2e, unlike IEEE journals/conferences, places
% % footnotes above bottom floats. This can be corrected via the
% % \fnbelowfloat command of the stfloats package.



% %%%%%%%%%%%%%%
% % Conclusion %
% %%%%%%%%%%%%%%
% \section{Conclusion} \label{sec:conclusion}

%     Our 800mm$^2$ design study seems to indicate that the best size for chiplets is somewhere between 40mm$^2$ and 80mm$^2$ for microprocessor logic and between 150mm$^2$ and 200mm$^2$ for random logic. Splitting a large design into chiplets improves yield substantially at first, but eventually, the cost and yield loss due to assembly begin to dominate.  Fast, low-cost, high-yielding assembly methods may help make many-chiplet systems practical just as high-yield die manufacturing processes can help make larger chips more practical. Although these two factors seem to have the greatest impact on the ideal chiplet size, it is also important to consider inter-chiplet IO requirements as splitting a design introduces the need for additional drivers for longer connecting wires along with ESD protection that increase both area and power usage. This impact can be minimized by assuring that manufacturing processes use ESD controls to reduce the ESD requirement on inter-chiplet IO cells. 

%     Further, due to brevity reasons, the case studies presented in this paper are limited and the models are general. Larger or smaller SoC sizes, mixed-size chiplet partitioning, models of NRE costs, and models of chiplet reuse are interesting future directions. Large ``minimum economically viable'' chiplet sizes have implications for a future chiplet-based design ecosystem. 40+mm$^2$ is a large real estate in advanced technology nodes making reusable chiplet IPs challenging. Our ongoing work is investigating these chiplet ecosystem challenges.




% % conference papers do not normally have an appendix


% % % use section* for acknowledgment
% % \section*{Acknowledgment}


% % The authors would like to thank...





% % trigger a \newpage just before the given reference
% % number - used to balance the columns on the last page
% % adjust value as needed - may need to be readjusted if
% % the document is modified later
% %\IEEEtriggeratref{8}
% % The "triggered" command can be changed if desired:
% %\IEEEtriggercmd{\enlargethispage{-5in}}

% % references section

% % can use a bibliography generated by BibTeX as a .bbl file
% % BibTeX documentation can be easily obtained at:
% % http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% % The IEEEtran BibTeX style support page is at:
% % http://www.michaelshell.org/tex/ieeetran/bibtex/
% %\bibliographystyle{IEEEtran}
% % argument is your BibTeX string definitions and bibliography database(s)
% %\bibliography{IEEEabrv,../bib/paper}
% %
% % <OR> manually copy in the resultant .bbl file
% % set second argument of \begin to the number of references
% % (used to reserve space for the reference number labels box)


% %%%%%%%%%%%%%%%%%%%%%
% % Temporary Section %
% %%%%%%%%%%%%%%%%%%%%%
% %\section{My Notes (Remove)}

%  %   All references that are not yet cited above listed here:
%   %    \cite{Prasad2017} \cite{Prasad2018} \cite{Das2004} \cite{Yang2001} \cite{Verplaetse2001} \cite{Stroobandt2000} \cite{Christie2000}
%    % \hl{remove}



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Bibliography and References %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Add references to references.bib document
% \bibliographystyle{savetrees}
% \bibliography{references, IEEEabrv}



% \end{document}
